Semi-Equivariant Conditional Normalizing Flows

We study the problem of learning conditional distributions of the form $p(G | \hat G)$, where $G$ and $\hat G$ are two 3D graphs, using continuous normalizing flows. We derive a semi-equivariance condition on the flow which ensures that conditional invariance to rigid motions holds. We demonstrate the effectiveness of the technique in the molecular setting of receptor-aware ligand generation.

==> floats/fig_model_illustration.tex <==
\begin{figure*}
    \centering
    \fig{illustration.pdf}{0.95}
    \caption{An illustration of the conditional probabilistic method. Top row: given a \receptor{} (on the leftmost side), denoted as $\hat{\mathcal{G}}$, we wish to conditionally sample a second 3D graph, which we refer to as the \ligand{} (represented by the enlarged vertices and edges),  denoted as $\mathcal{G}$. The Markov decomposition of the conditional distribution, which ultimately allows us to obtain the conditional probability $p(\mathcal{G} | \hat{\mathcal{G}})$, is illustrated by its successive stages from left to right. Specifically: $N$ is the number of vertices; $V$ is the list of vertices; $E$ is the list of edges; and $A$ is the set of global graph properties (light green marking). Bottom row: we illustrate the invariance to rigid motions applied jointly to both graphs and permutations applied to each of the graphs separately.}
    \label{fig:illustration}
\end{figure*}

==> old/data.tex <==
We use the same approach to evaluate the generative model as done in previous works \citep{ragoza2022generating, liu2022generating}. The reference evaluation set consists of 10 target receptors with each having multiple associated ligands, leading to 90 receptor-ligand pairs. After the previously described filtering procedure (Sec. \ref{sec:experiments}), 5 receptors remain corresponding to 27 receptor-ligand pairs. We complete the evaluation set, to yield 10 receptors corresponding to 90 pairs, by selecting data points from the validation set. These data points are chosen so that the ligands, receptors and pockets do not appear in the training set, and are not repeated in the evaluation set.

==> old/mathod_1.tex <==
\parbasic{Objective}
We refer to graphs whose vertices correspond to points in $\mathbb{R}^3$ as \textit{\graphtype{}s}.  We are given one \graphtype{}, which we refer to as the \textit{\receptor{}}, and which we denote $\recsym$; given this \receptor{}, we are then interested in learning about a second \graphtype{}, which we refer to as the \textit{\ligand{}}, and which we denote $\ligsym$.  In particular, we are interesting in learning a conditional distribution of the form $p(\ligsym | \recsym)$, which tells us which \ligand{}s match a given \receptor{}. In the molecular scenario, the \receptor{} will represent a receptor / target and the \ligand{} will represent a ligand; in the case of shape completion in computer vision, the \receptor{} will represent the part of the point cloud that we have been given, and the \ligand{} will represent the completion of this point cloud.
%One may think of the problem we wish to solve as a kind of graph completion, though we never actually construct a joint graph.

Note that to be physically plausible, the distribution $p(\ligsym | \recsym)$ must be invariant to certain groups of transformations: rigid motions applied jointly to both graphs, as well as permutations applied to each of the graphs separately.  Enforcing these invariances provides a strong inductive bias to our learning algorithm.

\parbasic{Organization}
This section proposes a method for learning such a conditional distribution $p(\ligsym | \recsym)$.  Section \ref{sec:notation} introduces notation.  Section \ref{sec:decomposition} decomposes the distribution into 4 subdistributions using a Markov decomposition, and shows how the invariance properties apply to each subdistribution.  Section \ref{sec:intermezzo} is an intermezzo, describing two types of Equivariant Graph Neural Networks (EGNNs); these EGNNs are then used in Sections \ref{sec:number} - \ref{sec:edge_and_properties} to propose forms for each of the subdistributions with the appropriate invariance properties.  The main result appears in Section \ref{sec:vertex}, which shows that the vertex subdistribution can be implemented as a particular type of continuous normalizing flow.

\subsection{Notation and Goal}
\label{sec:notation}

\parbasic{Notation} We use the following notation.  A \graphtype{} is given by
\begin{equation}
    \ligsym = (N, V, E, A)
\end{equation}
where $N$ is the number of vertices; $V$ is the list of vertices; $E$ is the list of edges; and $A$ is the set of global graph properties, i.e. properties which apply to the entire graph.  The vertex list\footnote{We use lists, rather than sets, so as to make the action of permutations clear.} is $V = \left( \mathbf{v}_i \right)_{i=1}^N$ where each vertex is specified by a vector $\mathbf{v}_i = (\mathbf{x}_i, \mathbf{h}_i)$; in which $\mathbf{x}_i \in \mathbb{R}^3$ is the position of the vertex, and $\mathbf{h}_i \in \mathbb{R}^{d_h}$ contains the properties of the vertex.  More generally, this may include continuous properties, discrete ordinal properties, and discrete categorical properties (using the one-hot representation); $\mathbf{h}_i$ may be thought of a concatenation of all such properties.  The edges in the graph $\ligsym$ are undirected, and the edge list $E$ is specified by a neighbourhood relationship.  Specifically, if $\eta_i$ is the set of vertex $i$'s neighbours, then we write $E = \left( \mathbf{e}_{ij} \right)_{i<j: j \in \eta_i}$.  The vector $\mathbf{e}_{ij} \in \mathbb{R}^{d_e}$ contains the properties of the edge connecting vertices $i$ and $j$; more generally, $\mathbf{e}_{ij}$ may contain a concatenation of various properties in a manner analogous to the vertex properties $\mathbf{h}_i$ as described above.  Finally, the graph properties are given by $K$ individual properties, i.e. $A = (\mathbf{a}_1, \dots, \mathbf{a}_K)$.  A given property $\mathbf{a}_k$ can be either continuous, categorical or ordinal. 

\parbasic{Rigid Transformations}  The action\footnote{
Note to the reader: other papers such as \cite{satorras2021flows} use the notation $E(n)$ rather than $E(3)$, as the transformation is applied to multiple atoms.  Here, we opt to use the notation $E(3)$, and $O(3)$ in the case of rotations, as there is a single transformation being applied to all of the atoms.  Our notation is made sensible and precise given the definitions in Equation (\ref{eq:rigid_action}) and the surrounding text.
}
of a rigid transformation $T \in E(3)$ on a graph $\ligsym$ is given by $T\ligsym = (TN, TV, TE, TA)$ where
\begin{equation}
    TV = \left( T\mathbf{v}_i \right)_{i=1}^N \quad \text{with} \quad T\mathbf{v}_i = (T\mathbf{x}_i, \mathbf{h}_i)
    \label{eq:rigid_action}
\end{equation}
and the other variables are unaffected by $T$; that is $TN = N$, $TE = E$, and $TA = A$.

\parbasic{Permutations} The action of a permutation $\pi \in \mathbb{S}_N$ on a graph $\ligsym$ with $N(\ligsym) = N$ is given by $\pi \ligsym = (\pi N, \pi V, \pi E, \pi A)$ where
\begin{equation}
    \pi V = \left( \mathbf{v}_{\pi_i} \right)_{i=1}^N \quad\quad \text{and} \quad\quad
    \pi E = \left( \mathbf{e}_{\pi_i\pi_j} \right)_{i<j: j \in \eta_i}
    \label{eq:permutation_action}
\end{equation}
and the other variables are unaffected by $\pi$; that is, $\pi N = N$ and $\pi A = A$.

\parbasic{Goal} We assume that we have both a \receptor{} and a \ligand{}, each of which is specified by a \graphtype{}.  We denote
\begin{equation}
    \ligsym = (N, V, E, A) = \text{\ligand{}} \quad \quad \text{and} \quad \quad \recsym = (\hat{N}, \hat{V}, \hat{E}, \hat{A}) = \text{\receptor{}}
\end{equation}
(Note: if there properties of the entire \complex{} consisting of both the \receptor{} and the \ligand{}, these are subsumed into the \ligand{} properties, $A$.)  Our goal is to learn a conditional generative model: given the \receptor{}, we would like to generate possible \ligand{}s.  Formally, we want to learn
\begin{equation}
    p(\ligsym | \recsym)
\end{equation}
We want our generative model to observe two types of symmetries.  First, if we transform both the \ligand{} and the \receptor{} with the same rigid transformation, the probability should not change:
\begin{equation}
    p(T\ligsym | T\recsym) = p(\ligsym | \recsym) \quad \text{for all } T \in E(3)
    \label{eq:invariance_rigid}
\end{equation}
Second, permuting the order of either the \ligand{} or the \receptor{} should not affect the probability:
\begin{equation}
    p(\pi \ligsym | \hat{\pi} \recsym) = p(\ligsym | \recsym) \quad \text{for all } \pi \in \mathbb{S}_{N}, \, \hat{\pi} \in \mathbb{S}_{\hat{N}}
    \label{eq:invariance_permutation}
\end{equation}

\subsection{Decomposition of the Conditional Distribution and Invariance Properties}
\label{sec:decomposition}

\parbasic{Decomposition} We may breakdown the conditional generative model as follows:
\begin{equation}
    p(\ligsym | \recsym) = p(N, V, E, A | \recsym) = p(N | \recsym) \, \cdot \, p(V | N, \recsym) \, \cdot \, p(E| N, V, \recsym) \, \cdot \, p(A | N, V, E, \recsym)
    \label{eq:markov}
\end{equation}
We refer the four terms on the right-hand side of the equation as the Number Distribution, the Vertex Distribution, the Edge Distribution, and the Property Distribution, respectively.  We will specify a model for each of these distributions in turn.  First, however, we examine how the invariance properties affect the distributions.  

\parbasic{Invariance Properties} Using the relations for rigid body transformations in (\ref{eq:rigid_action}), we have that 
\begin{equation}
    p(T\ligsym | T\recsym) = p(N | T\recsym) \, \cdot \, p(TV | N, T\recsym) \, \cdot \, p(E| N, TV, T\recsym) \, \cdot \, p(A | N, TV, E, T\recsym)
    \label{eq:markov_with_rigid}
\end{equation}
Similarly, using the relations for permutations in (\ref{eq:permutation_action}), we have that
\begin{align}
    p(\pi \ligsym | \hat{\pi} \recsym) = p(N | \hat{\pi} \recsym) \, \cdot \, p(\pi V | N, \hat{\pi} \recsym) \, \cdot \, p(\pi E| N, \pi V, \hat{\pi} \recsym) \, \cdot \, p(A | N, \pi V, \pi E, \hat{\pi} \recsym) 
    \label{eq:markov_with_permutation}
\end{align}


Comparing Equation (\ref{eq:markov}) with (\ref{eq:markov_with_rigid}) and (\ref{eq:markov_with_permutation}), the following conditions are sufficient for conditional rigid body invariance (\ref{eq:invariance_rigid}) and conditional permutation invariance (\ref{eq:invariance_permutation}):
\begin{align}
    & p(N | T\recsym) = p(N | \recsym)
    & & p(N | \hat{\pi} \recsym) = p(N | \recsym) \label{eq:number_invariance} \\
    & p(TV | N, T\recsym) = p(V | N, \recsym) 
    & & p(\pi V | N, \hat{\pi} \recsym) = p(V | N, \recsym) \label{eq:vertex_invariance} \\
    & p(E| N, TV, T\recsym) = p(E| N, V, \recsym) 
    & & p(\pi E| N, \pi V, \hat{\pi} \recsym) = p(E| N, V, \recsym) \label{eq:edge_invariance} \\
    & p(A | N, TV, E, T\recsym) = p(A | N, V, E, \recsym) \quad
    & & p(A | N, \pi V, \pi E, \hat{\pi} \recsym) = p(A | N, V, E, \recsym) \label{eq:property_invariance}
\end{align}

The conditional probabilistic approach is illustrated in Figure \ref{fig:illustration}.
\input{floats/fig_model_illustration}

\subsection{Intermezzo: Two Flavours of EGNNs}
\label{sec:intermezzo}

In order to incorporate the relevant invariance properties, it will be helpful to use Equivariant Graph Neural Networks, also known as EGNNs \citep{satorras2021egnn}.  We now introduce two separate flavours of EGNNs, one which applies to the \receptor{} alone, and a second which applies to the combination of the \receptor{} and the \ligand{}.

\parbasic{\titlecap{\receptor{}} EGNN} \label{sec:receptor_egnn}
This is the standard EGNN which is described in \citep{satorras2021egnn}, applied to the \receptor{}.  As we are dealing with the \receptor{} we use hatted variables:
\begin{align}
    & \bh{m}^\ell_{ij} = \hat{\phi}_e(\bh{h}^\ell_i, \bh{h}^\ell_j, \|\bh{x}^\ell_i-\bh{x}^\ell_j\|^2, \|\bh{x}^0_i-\bh{x}^0_j\|^2, \bh{e}_{ij}, \{\bh{a}_k\})
    \hspace{0.65cm}
    \hat{b}_{ij}^\ell = \sigma(\hat{\phi}_b(\bh{m}_{ij}^\ell))
    \hspace{0.55cm}
    \bh{m}_i^\ell  = \sum_{j \in \hat{\eta}_i} \hat{b}_{ij}^\ell \bh{m}_{ij}^\ell
    \notag \\
    & \bh{x}^{\ell+1}_i=\bh{x}^\ell_i+\left(\sum_{j\neq i} {\frac{(\bh{x}^\ell_i-\bh{x}^\ell_j)}{\|\bh{x}^\ell_i-\bh{x}^\ell_j\|+1}} \right) \hat{\phi}_x(\bh{m}^\ell_{ij})
    \hspace{1.7cm}
    \bh{h}^{\ell+1}_i=\bh{h}^{\ell}_i + \hat{\phi}_h(\bh{h}^\ell_i,\bh{m}^\ell_i)
\end{align}
The particular \titlecap{\receptor{}} EGNN is thus specified by the functions $\hat{\phi}_e, \hat{\phi}_b, \hat{\phi}_x, \hat{\phi}_h$. In practice, prior to applying the EGNN one may apply: (i) an ActNorm layer to the atom positions and features, as well as the edge features and graph features; (ii) a linear transformation to the atom properties.

\parbasic{\conditionalEGNN{}}
It is possible to design a joint EGNN on the \receptor{} and the \ligand{}, by constructing a single graph to capture both.  The main problem with this approach is that in many applications, the \receptor{} can be much larger than the \ligand{}; for example, in the molecular scenario the receptor is 1-2 orders of magnitude larger than the ligand.  As a result, this naive approach will lead to a situation in which the \ligand{} is ``drowned out'' by the \receptor{}, making it difficult to learn about the \ligand{}.

We therefore take a different approach: we compute summary signatures of the \receptor{} based on the \titlecap{\receptor{}} EGNN, and use these as input to a \titlecap{\ligand{}} EGNN.  Our signatures will be based on the feature variables $\bh{h}^\ell_j$ from each layer $\ell = 1, \dots, \hat{L}$.  These variables are invariant to rigid body transformations by construction; furthermore, we can introduce permutation invariance by averaging, that is $\bh{h}^\ell_{av} = \frac{1}{\hat{N}} \sum_{j=1}^{\hat{N}} \bh{h}^\ell_j$.
In Section \ref{sec:vertex}, we will see that the vertex distribution is described by a continuous normalizing flow.  In anticipation of this, we wish to introduce a dependence (crucial in practice) on the time variable $t$ of the ODE corresponding to this flow.  Thus, the \receptor{} at layer $\ell$ of the \ligand{}'s EGNN is summarized by the signature $\bh{g}^\ell$ which depends on both $\{ \bh{h}^\ell_{av} \}$ and $t$:
\begin{equation}
    \bh{g}^0 = \phi^0_g \left( \bh{h}^1_{av}, \dots, \bh{h}^{\hat{L}}_{av}, t \right) \qquad \text{and} \qquad
    \bh{g}^\ell = \phi^\ell_g \left( \bh{g}^{\ell-1} \right) \quad \ell = 1, \dots, L
\end{equation}
%Note that there are $L+1$ separate functions $\{ \phi^\ell_g \}_{\ell=0}^L$.

These invariant \receptor{} signatures $\{ \bh{g}^\ell \}_{\ell=1}^L$ are then naturally incorporated into the \conditionalEGNN{} as follows:
\begin{align}
    & \mathbf{m}^\ell_{ij} = \phi_e\left(\mathbf{h}^\ell_i,\mathbf{h}^\ell_j,  \|\mathbf{x}^\ell_i-\mathbf{x}^\ell_j\|^2, \|\mathbf{x}^0_i-\mathbf{x}^0_j\|^2 , \bh{g}^\ell, t \right)
    \hspace{0.5cm}
    \quad b_{ij}^\ell = \sigma(\phi_b(\mathbf{m}_{ij}^\ell, \bh{g}^\ell ))
    \hspace{0.5cm}
    \mathbf{m}^\ell_i  = \sum_{j=1}^N b^\ell_{ij} \mathbf{m}^\ell_{ij}
    \notag \\
    & \mathbf{x}^{\ell+1}_i= \mathbf{x}^\ell_i + \left( \sum_{j\neq i} {\frac{(\mathbf{x}^\ell_i-\mathbf{x}^\ell_j)}{\|\mathbf{x}^\ell_i-\mathbf{x}^\ell_j\|+1}} \right) \phi_x(\mathbf{m}^\ell_{ij} , \bh{g}^\ell )
    \hspace{0.7cm}
    \mathbf{h}^{\ell+1}_i = \mathbf{h}^{\ell}_i + \phi_h(\mathbf{h}^\ell_i, \mathbf{m}^\ell_i , \bh{g}^\ell )
\end{align}
The particular \conditionalEGNN{} is thus specified by the functions $\{ \phi^\ell_g \}_{\ell=0}^L, \phi_e, \phi_b, \phi_x, \phi_h$.

\subsection{The Number Distribution: $p(N | \recsym)$}
\label{sec:number}

\parbasic{Construction} Given the invariance conditions for the number distribution $p(N | \recsym)$ described in Equation (\ref{eq:number_invariance}), we propose the following distribution.  Let $\boldsymbol{\zeta}_N$ indicate a one-hot vector, where the index corresponding to $N$ is filled in with a $1$.  Based on the output of the \receptor{} EGNN, compute
\begin{equation}
    p(N | \recsym) = \boldsymbol{\zeta}_N^T \texttt{MLP}' \left( \frac{1}{\hat{N}} \sum_{i=1}^{\hat{N}} \texttt{MLP} \left( \bh{h}^L_i \right) \right)
\end{equation}
where the outer $\texttt{MLP}$'s (multilayer perceptron) last layer is a softmax of size equal to the maximum number of atoms allowed.

Due to the fact that we use the $\bh{h}^L_i$ vectors (and not the $\bh{x}^L_i$ vectors), we have the first invariance condition, as $T\bh{h}^L_i = \bh{h}^L_i$.  Due to the fact that we use an average, we have the second invariance condition.  Note that we can choose to make the inner $\texttt{MLP}$ the identity, if we so desire.

\parbasic{Loss Function}  The loss function is straightforward here -- it is simply the negative log-likelihood of the number distribution, i.e. $L(\theta) = \mathbb{E}_{\ligsym, \recsym} \left[ -\log p(N | \recsym; \theta) \right]$.

\subsection{The Vertex Distribution: $p(V | N, \recsym)$ via Continuous Normalizing Flows}
\label{sec:vertex}

\parbasic{General Notation} Given the invariance conditions for the vertex distribution $p(V | N, \recsym)$ described in Equation (\ref{eq:vertex_invariance}), we now outline a procedure for constructing such a distribution.  We begin with some notation.  Let us define a vectorization operation on the vertex list $V$, which produces a vector $\mathbf{v}$; we refer to this as a \textit{vertex vector}.  Recall that $V = (\mathbf{v}_i)_{i=1}^N$ where $\mathbf{v}_i = (\mathbf{x}_i, \mathbf{h}_i)$.  Let
\begin{equation}
    \mathbf{x} = \texttt{concat}(\mathbf{x}_1, \dots, \mathbf{x}_N) 
    \hspace{0.8cm}
    \mathbf{h} = \texttt{concat}(\mathbf{h}_1, \dots, \mathbf{h}_N)
    \hspace{0.8cm}
    \mathbf{v} = \texttt{concat}(\mathbf{x}, \mathbf{h})
\end{equation}
The vertex vector $\mathbf{v} \in \mathbb{R}^{d_v^N}$ where $d_v^N = (d_h+3)N$. We denote the mapping from the vertex list $V$ to the vertex vector $\mathbf{v}$ as the vectorization operation $\texttt{vec}(\cdot)$:
\begin{equation}
    \mathbf{v} = \texttt{vec}(V) \quad \quad \text{ and } \quad \quad V = \texttt{vec}^{-1}(\mathbf{v})
\end{equation}
We have already described the action of rigid body transformation $T$ and permutations $\pi$ on the vertex list $V$ in Equations (\ref{eq:rigid_action}) and (\ref{eq:permutation_action}).  It is easy to extend this to vertex vectors $\mathbf{v}$ using the \texttt{vec} operation; we have $T\mathbf{v} = \texttt{vec}( T\texttt{vec}^{-1}(\mathbf{v}) )$ and $\pi\mathbf{v} = \texttt{vec}( \pi\texttt{vec}^{-1}(\mathbf{v}) )$.
% \begin{equation}
%     T\mathbf{v} = \texttt{vec}\left( T\texttt{vec}^{-1}(\mathbf{v}) \right) \quad \quad \text{and} \quad \quad
%     \pi\mathbf{v} = \texttt{vec}\left( \pi\texttt{vec}^{-1}(\mathbf{v}) \right)
% \end{equation}

Given the above, it is sufficient for us to describe the distribution $p_{vec}(\mathbf{v} | \recsym)$
from which the vertex distribution $p(V | N, \recsym)$ follows directly, $p(V | N, \recsym) = p_{vec}(\texttt{vec}(V) | \recsym)$.  Note that we have suppressed $N$ in the condition in $p_{vec}(\cdot)$, as $\mathbf{v}$ is a vector of dimension $d_v^N$, so the $N$ dependence is already implicitly encoded.  

\parbasic{\ccmapping{} and Semi-Equivariance} Let $\gamma$ be a function which takes as input the \complex{} consisting of both the \ligand{} $\ligsym$ and \receptor{} $\recsym$, and outputs a new vertex list $V'$ for the \ligand{} $\ligsym$:
\begin{equation}
    \quad V' = \gamma(\ligsym, \recsym)
\end{equation}
We refer to $\gamma$ as a \textit{\ccmapping{}}.  A rigid body transformation $T \in E(3)$ consists of a rotation and translation; let the rotation be denoted as $T_{rot}$.  Then we say that $\gamma$ is \textit{rotation semi-equivariant} if
\begin{equation}
    \gamma(T_{rot}\ligsym, T\recsym) = T_{rot}\gamma(\ligsym, \recsym) \quad \text{for all } T \in E(3)
\end{equation}
where, as before, the action of $T$ on a graph is given by Equation (\ref{eq:rigid_action}).  $\gamma$ is said to be \textit{permutation semi-equivariant} if
\begin{equation}
    \gamma(\pi \ligsym, \hat{\pi}\recsym) = \pi \gamma(\ligsym, \recsym) \quad \text{for all } \pi \in \mathbb{S}_N \text{ and } \hat{\pi} \in \mathbb{S}_{\hat{N}}
    \label{eq:gamma_permutation}
\end{equation}
where, as before, the action of the permutation on a graph is given by Equation (\ref{eq:permutation_action}).  Note in the definitions of both types of semi-equivariance, the differing roles played by the \ligand{} and \receptor{}; as the equivariant behaviour only applies to the \ligand{}, we have used the term semi-equivariance.

\parbasic{\conditionalFlow{}} Let $\gamma$ be a \ccmapping{}.  If $\mathbf{v}$ is a vertex vector, define $\ligsym_{\mathbf{v}}$ to be the graph $\ligsym$ with the vertex set replaced by $\texttt{vec}^{-1}(\mathbf{v})$. Then the following ordinary differential equation is referred to as a \textit{\conditionalFlow{}}:
\begin{equation}
    \frac{d\mathbf{u}}{dt} = \texttt{vec}\left( \gamma(\ligsym_{\mathbf{u}} , \recsym) \right), \quad \text{with } \mathbf{u}(0) = \mathbf{z}
\end{equation}
where the initial condition $\mathbf{z} \sim \mathcal{N}(0, \mathbf{I})$ is a Gaussian random vector of dimension $d_v^N$, and the ODE is run until $t=1$.  $\mathbf{u}(1)$ is thus the output of the \conditionalFlow{}.

\parbasic{Vertex Distributions with Appropriate Invariance} We now have all of the necessary ingredients in order to construct a distribution $p_{vec}(\mathbf{v} | \recsym)$ which yields a vertex distribution $p(V | N, \recsym)$ that satisfies the invariance conditions that we require.  The following is our main result:

\begin{theorem}[Invariant Vertex Distribution]
Let $\mathbf{u}(1)$ be the output of a \conditionalFlow{} specified by the \ccmapping{} $\gamma$.  Let the mean position of the \receptor{} be given by $\bh{x}_{av} = \frac{1}{\hat{N}} \sum_{i=1}^{\hat{N}} \bh{x}_i$, and define the following quantities
\begin{equation}
    \alpha = \frac{N}{N + \hat{N}} \quad \quad
    \Omega_{\recsym} = 
    \begin{bmatrix}
        \mathbf{I}_{3N} - \frac{\alpha}{N} \mathbf{1}_{N \times N} \otimes \mathbf{I}_3 & \mathbf{0} \\
        \mathbf{0} & \mathbf{I}_{d_h N}
    \end{bmatrix}
    \quad \quad
    \omega_{\recsym} = 
    \begin{bmatrix}
        -(1-\alpha) \mathbf{1}_{N \times 1} \otimes \bh{x}_{av} \\
        \mathbf{0}
    \end{bmatrix}
\end{equation}
where $\otimes$ indicates the Kronecker product.  Finally, let 
\begin{equation}
    \mathbf{v} = \Omega_{\recsym}^{-1} \left( \mathbf{u}(1) - \omega_{\recsym} \right)
\end{equation}

Suppose that $\gamma$ is both rotation semi-equivariant and permutation semi-equivariant.  Then the resulting distribution on $\mathbf{v}$, that is $p_{vec}(\mathbf{v} | \recsym)$, yields a vertex distribution $p(V | N, \recsym) = p_{vec}(\texttt{vec}(V) | \recsym)$ that satisfies the invariance conditions in Equation (\ref{eq:vertex_invariance}).
\end{theorem}

\textbf{\textit{Proof:}} See Section \ref{sec:proof}.

\parbasic{Designing the \ccmapping{}} Examining the theorem, we see that the one degree of freedom that we have is the \ccmapping{} $\gamma$.  For this, we choose to use the \conditionalEGNN{}, where the output of the \ccmapping{} $V' = \gamma(\ligsym, \recsym)$ can simply be the final layer, i.e. the $i^{th}$ vertex of $V'$ is given by $v'_i = (\mathbf{x}_i^L, \mathbf{h}_i^L)$.  In practice, we use a slightly modified version of the foregoing, in which we displace the coordinates of the final layer by the initial input coordinates to the EGNN, that is $v'_i = (\mathbf{x}_i^L-\mathbf{x}_i, \mathbf{h}_i^L)$.  We have found the latter to converge well empirically.

The rotation semi-equivariance of $\gamma$ (both versions - ordinary and displaced) follows straightforwardly from the rotation semi-equivariance of EGNNs and the rotation invariance of the \receptor{} signatures $\{ \bh{g}^\ell \}_{\ell=1}^L$.  Similarly, the permutation semi-equivariance follows from the permutation semi-equivariance of EGNNs and the permutation invariance of the \receptor{} signatures.

\parbasic{Loss Function}  The vertex distribution is described by a continuous normalizing flow.  The loss function and its optimization are implemented using standard techniques from this field \citep{chen2018neural,grathwohl2018ffjord,chen2018continuous}.  As the feature vectors can contain discrete variables such as the atom type, then techniques based on variational dequantization \citep{ho2019flow++} and argmax flows \cite{hoogeboom2021argmax} can be used, for ordinal and categorical features respectively.  This is parallel to the treatment in \citep{satorras2021flows}.

\subsection{Extensions: The Edge and Properties Distributions}
\label{sec:edge_and_properties}

We now outline methods for computing the Edge and Properties Distributions.  In practice, we do not implement these methods, but rather use a standard simple technique based on inferring edge properties directly from vertices, see Section \ref{sec:experiments}.  Nevertheless, we describe these methods for completeness.

\parbasic{The Edge Distribution} Given the invariance conditions for the edge distribution $p(E| N, V, \recsym)$ described in Equation (\ref{eq:edge_invariance}), we propose
% the following distribution:  
% \begin{equation}
%     p\left( E = \left( \mathbf{e}_{ij} \right)_{i<j: j \in \eta_i} | N, V, \recsym \right) = 
%     \prod_{i<j: j \in \eta_i} p\left( \mathbf{e}_{ij} | N, V, \recsym \right)
% \end{equation}
% In other words, the distribution of edges displays \textit{conditional independence}.  
a distribution which displays \textit{conditional independence}: 
$p\left( E = ( \mathbf{e}_{ij} \right)_{i<j: j \in \eta_i} | N, V, \recsym ) = 
    \prod_{i<j: j \in \eta_i} p( \mathbf{e}_{ij} | N, V, \recsym )$.
We opt for conditional independence for two reasons: (1) The usual Markov decomposition of the probability distribution with terms of the form $p( \mathbf{e}_{ij} | \mathbf{e}_{<ij}, N, V, \recsym )$ implies a particular ordering of the edges, and is therefore not permutation-invariant. (2) $V$ is a deterministic and invertible function of the flow's noise vector $\mathbf{z}$; thus, conditioning on $V$ is the same as conditioning on $\mathbf{z}$.  If $E$ is a deterministic (but not necessarily invertible) function of $\mathbf{z}$, then conditional independence is correct.

To compute $p( \mathbf{e}_{ij} | N, V, \recsym )$, we use a second \conditionalEGNN{}.  The key distinction between this network and the \conditionalEGNN{} used in computing the vertex distribution is the initial conditions.  In the case of the vertex distribution, the initial conditions are $\mathbf{x}_i^1 = \mathbf{0}$ and $\mathbf{h}_i^1 = \mathbf{0}$.  In the current case of the edge distribution, we are given $V$ (we are conditioning on it); thus, we take the initial conditions to be $\bt{x}_i^1 = \mathbf{x}_i(V)$ and $\bt{h}_i^1 = \mathbf{h}_i(V)$.  In other words, the initial values are given the vertex list $V$ itself.

Given this second \conditionalEGNN{}, we can compute the edge distribution as
\begin{equation}
    p\left( \mathbf{e}_{ij} | N, V, \recsym \right) = \mathbf{e}_{ij}^T \, \texttt{MLP}\left(\bt{m}^L_{ij}\right)
\end{equation}
in the case of categorical properties (where $\texttt{MLP}$'s output is a softmax with $d_e$ entries); analogous expressions exist for ordinal or continuous properties.  It is straightforward to see that this distribution satisfies the invariance properties in Equation (\ref{eq:edge_invariance}).  The corresponding loss function is a simple cross-entropy loss (or regression loss for non-categorical properties).

\parbasic{The Property Distribution} Given the invariance conditions for the property distribution $p(A | N, V, E, \recsym)$ described in Equation (\ref{eq:property_invariance}), we propose the following distribution.  We use a standard Markov decomposition:
$
    p(A | N, V, E, \recsym) = \prod_{k=1}^K p\left( \mathbf{a}_k | \mathbf{a}_{1:(k-1)}, N, V, E, \recsym \right)
$.
Let
\begin{equation}
    \boldsymbol{\xi}_h = \frac{1}{N} \sum_{i=1}^N \texttt{MLP} \left( \bt{h}^L_i \right)
    \hspace{0.8cm}
    \boldsymbol{\xi}_e = \frac{1}{|E|} \sum_{i<j: j \in \eta_i} \texttt{MLP} \left( \mathbf{e}_{ij} \right)
    \hspace{0.8cm}
    \boldsymbol{\xi}_{a,k} = \texttt{MLP}\left( \sum_{j=1}^{k-1} W_j \mathbf{a}_j \right)
\end{equation}
where the matrices $W_1, \dots W_K$ all have the same number of rows.
Then we set
\begin{equation}
    p\left( \mathbf{a}_k \left| \mathbf{a}_{1:(k-1)}, N, V, E, \recsym \right. \right) = \mathbf{a}_k^T \texttt{MLP} \left( \texttt{concat}\left( \boldsymbol{\xi}_h , \boldsymbol{\xi}_e, \boldsymbol{\xi}_{a,k} \right) \right)
\end{equation}
in the case of categorical properties; analogous expressions exist for ordinal or continuous properties.  Note that the only item which changes for the different properties $k$ is the vector $\boldsymbol{\xi}_{a,k}$. It is easy to see that this distribution satisfies the invariance properties in Equation (\ref{eq:property_invariance}).  The corresponding loss function is a simple cross-entropy loss (or regression loss for non-categorical properties).


==> old/method_2.tex <==
\subsection{Notation and Goal}
\label{sec:notation}

\parbasic{Notation} A \graphtype{} is given by $\ligsym = (N, V, E, A)$, where $N$ is the number of vertices; $V$ is the list of vertices; $E$ is the list of edges; and $A$ is the set of global graph properties, i.e. properties which apply to the entire graph.  The vertex list\footnote{We use lists, rather than sets, so as to make the action of permutations clear.} is $V = \left( \mathbf{v}_i \right)_{i=1}^N$ where each vertex is specified by a vector $\mathbf{v}_i = (\mathbf{x}_i, \mathbf{h}_i)$; in which $\mathbf{x}_i \in \mathbb{R}^3$ is the position of the vertex, and $\mathbf{h}_i \in \mathbb{R}^{d_h}$ contains the properties of the vertex.  The edges in the graph $\ligsym$ are undirected, and the edge list $E$ is specified by a neighbourhood relationship.  Specifically, if $\eta_i$ is the set of vertex $i$'s neighbours, then we write $E = \left( \mathbf{e}_{ij} \right)_{i<j: j \in \eta_i}$.  The vector $\mathbf{e}_{ij} \in \mathbb{R}^{d_e}$ contains the properties of the edge connecting vertices $i$ and $j$.  Finally, the graph properties are given by $K$ individual properties, i.e. $A = (\mathbf{a}_1, \dots, \mathbf{a}_K)$. 

\parbasic{Rigid Transformations}  The action of a rigid transformation $T \in E(3)$ on a graph $\ligsym$ is given by $T\ligsym = (TN, TV, TE, TA)$ where $TV = \left( T\mathbf{v}_i \right)_{i=1}^N$ with $T\mathbf{v}_i = (T\mathbf{x}_i, \mathbf{h}_i)$.  The other variables are unaffected by $T$; that is $TN = N$, $TE = E$, and $TA = A$.

\parbasic{Permutations} The action of a permutation $\pi \in \mathbb{S}_N$ on a graph $\ligsym$ with $N(\ligsym) = N$ is given by $\pi \ligsym = (\pi N, \pi V, \pi E, \pi A)$ where $\pi V = \left( \mathbf{v}_{\pi_i} \right)_{i=1}^N$ and $\pi E = \left( \mathbf{e}_{\pi_i\pi_j} \right)_{i<j: j \in \eta_i}$.  The other variables are unaffected by $\pi$; that is, $\pi N = N$ and $\pi A = A$.

\parbasic{Goal} We assume that we have both a \receptor{} and a \ligand{}, each of which is specified by a \graphtype{}.  We denote the \receptor{} as $\recsym = (\hat{N}, \hat{V}, \hat{E}, \hat{A})$ and the \ligand{} as $\ligsym = (N, V, E, A)$.  Our goal is to learn a conditional generative model: given the \receptor{}, we would like to generate possible \ligand{}s.  Formally, we want to learn $p(\ligsym | \recsym)$. We want our generative model to respect two types of symmetries, expressed mathematically as:
\begin{equation}
    p(T\ligsym | T\recsym) = p(\ligsym | \recsym) \,\, \forall T \in E(3) 
    \quad \text{and} \quad
    p(\pi \ligsym | \hat{\pi} \recsym) = p(\ligsym | \recsym) \,\, \forall \pi \in \mathbb{S}_{N}, \, \hat{\pi} \in \mathbb{S}_{\hat{N}}
    \label{eq:invariance}
\end{equation}
The first condition says that if we transform both the \ligand{} and the \receptor{} with the same rigid transformation, the probability should not change.  The second condition says that permuting the order of either the \ligand{} or the \receptor{} should not affect the probability.

\parbasic{General Approach}  We design our generative model $p(\ligsym | \recsym)$ by using a Markov decomposition:
\begin{equation}
    p(\ligsym | \recsym) = p(N, V, E, A | \recsym) = p(N | \recsym) \, \cdot \, p(V | N, \recsym) \, \cdot \, p(E| N, V, \recsym) \, \cdot \, p(A | N, V, E, \recsym)
    \label{eq:markov}
\end{equation}
In this paper, we focus on the first two terms on the right-hand side of the equation, which we refer to as the Number Distribution and the Vertex Distribution.  The latter two terms may also be specified in a relatively straightforward fashion, but are not the focus of our investigation in this paper.

\subsection{Two Flavours of EGNNs}
\label{sec:intermezzo}

In order to incorporate the relevant invariance properties, it will be helpful to use Equivariant Graph Neural Networks, also known as EGNNs \citep{satorras2021egnn}.  We now introduce two separate flavours of EGNNs, one which applies to the \receptor{} alone, and a second which applies to the combination of the \receptor{} and the \ligand{}.

\parbasic{\titlecap{\receptor{}} EGNN} \label{sec:receptor_egnn}
This is the standard EGNN which is described in \citep{satorras2021egnn}, applied to the \receptor{}. The particular \titlecap{\receptor{}} EGNN is detailed in Section \ref{sec:egnn_models} and specified by the functions $\hat{\phi}_e, \hat{\phi}_b, \hat{\phi}_x, \hat{\phi}_h$. As we are dealing with the \receptor{} we use hatted variables.

\parbasic{\conditionalEGNN{}}
It is possible to design a joint EGNN on the \receptor{} and the \ligand{}, by constructing a single graph to capture both.  The main problem with this approach is that in many applications, the \receptor{} can be much larger than the \ligand{}; for example, in the molecular scenario the receptor is 1-2 orders of magnitude larger than the ligand.  As a result, this naive approach will lead to a situation in which the \ligand{} is ``drowned out'' by the \receptor{}, making it difficult to learn about the \ligand{}. We therefore take a different approach: we compute summary signatures of the \receptor{} based on the \titlecap{\receptor{}} EGNN, and use these as input to a \titlecap{\ligand{}} EGNN.  Our signatures will be based on the feature variables $\bh{h}^\ell_j$ from each layer $\ell = 1, \dots, \hat{L}$.  These variables are invariant to rigid body transformations by construction; furthermore, we can introduce permutation invariance by averaging, that is $\bh{h}^\ell_{av} = \frac{1}{\hat{N}} \sum_{j=1}^{\hat{N}} \bh{h}^\ell_j$.
In Section \ref{sec:vertex}, we will see that the vertex distribution is described by a continuous normalizing flow.  In anticipation of this, we wish to introduce a dependence (crucial in practice) on the time variable $t$ of the ODE corresponding to this flow.  Thus, the \receptor{} at layer $\ell$ of the \ligand{}'s EGNN is summarized by the signature $\bh{g}^\ell$ which depends on both $\{ \bh{h}^\ell_{av} \}$ and $t$:
\begin{equation}
    \bh{g}^0 = \phi^0_g \left( \bh{h}^1_{av}, \dots, \bh{h}^{\hat{L}}_{av}, t \right) \qquad \text{and} \qquad
    \bh{g}^\ell = \phi^\ell_g \left( \bh{g}^{\ell-1} \right) \quad \ell = 1, \dots, L
\end{equation}

These invariant \receptor{} signatures $\{ \bh{g}^\ell \}_{\ell=1}^L$ are then naturally incorporated into the \conditionalEGNN{} as detailed in Section \ref{sec:egnn_models}. The particular \conditionalEGNN{} is thus specified by the functions $\{ \phi^\ell_g \}_{\ell=0}^L, \phi_e, \phi_b, \phi_x, \phi_h$.

\subsection{The Number Distribution: $p(N | \recsym)$}
\label{sec:number}

\parbasic{Construction} Given the invariance conditions described in Equation (\ref{eq:invariance}), we propose the following distribution.  Let $\boldsymbol{\zeta}_N$ indicate a one-hot vector, where the index corresponding to $N$ is filled in with a $1$.  Based on the output of the \receptor{} EGNN, compute
% \begin{equation}
%     p(N | \recsym) = \boldsymbol{\zeta}_N^T \texttt{MLP}' \left( \frac{1}{\hat{N}} \sum_{i=1}^{\hat{N}} \texttt{MLP} \left( \bh{h}^L_i \right) \right)
% \end{equation}
\begin{equation}
    p(N | \recsym) = \boldsymbol{\zeta}_N^T \texttt{MLP}' \left( \Sigma_{i=1}^{\hat{N}} \texttt{MLP} ( \bh{h}^L_i ) /  \hat{N} \right) 
\end{equation}
where the outer $\texttt{MLP}$'s (multilayer perceptron) last layer is a softmax of size equal to the maximum number of atoms allowed.

Due to the fact that we use the $\bh{h}^L_i$ vectors (and not the $\bh{x}^L_i$ vectors), we have the first invariance condition, as $T\bh{h}^L_i = \bh{h}^L_i$.  Due to the fact that we use an average, we have the second invariance condition.  Note that we can choose to make the inner $\texttt{MLP}$ the identity, if we so desire.

\parbasic{Loss Function}  The loss function is straightforward here -- it is simply the negative log-likelihood of the number distribution, i.e. $L(\theta) = \mathbb{E}_{\ligsym, \recsym} [ -\log p(N | \recsym; \theta) ]$.

\subsection{The Vertex Distribution: $p(V | N, \recsym)$ via Continuous Normalizing Flows}
\label{sec:vertex}

\parbasic{General Notation} Define a vectorization operation on the vertex list $V$, which produces a vector $\mathbf{v}$; we refer to this as a \textit{vertex vector}.  Recall that $V = (\mathbf{v}_i)_{i=1}^N$ where $\mathbf{v}_i = (\mathbf{x}_i, \mathbf{h}_i)$.  Let
\begin{equation}
    \mathbf{x} = \texttt{concat}(\mathbf{x}_1, \dots, \mathbf{x}_N) 
    \hspace{0.8cm}
    \mathbf{h} = \texttt{concat}(\mathbf{h}_1, \dots, \mathbf{h}_N)
    \hspace{0.8cm}
    \mathbf{v} = \texttt{concat}(\mathbf{x}, \mathbf{h})
\end{equation}
The vertex vector $\mathbf{v} \in \mathbb{R}^{d_v^N}$ where $d_v^N = (d_h+3)N$. We denote the mapping from the vertex list $V$ to the vertex vector $\mathbf{v}$ as the vectorization operation $\texttt{vec}(\cdot)$: we write $\mathbf{v} = \texttt{vec}(V)$ and $V = \texttt{vec}^{-1}(\mathbf{v})$.
% \begin{equation}
%     \mathbf{v} = \texttt{vec}(V) \quad \quad \text{ and } \quad \quad V = \texttt{vec}^{-1}(\mathbf{v})
% \end{equation}
We have already described the action of rigid body transformation $T$ and permutations $\pi$ on the vertex list $V$ in Section \ref{sec:notation}.  It is easy to extend this to vertex vectors $\mathbf{v}$ using the \texttt{vec} operation; we have $T\mathbf{v} = \texttt{vec}( T\texttt{vec}^{-1}(\mathbf{v}) )$ and $\pi\mathbf{v} = \texttt{vec}( \pi\texttt{vec}^{-1}(\mathbf{v}) )$.

Given the above, it is sufficient for us to describe the distribution $p_{vec}(\mathbf{v} | \recsym)$
from which the vertex distribution $p(V | N, \recsym)$ follows directly, $p(V | N, \recsym) = p_{vec}(\texttt{vec}(V) | \recsym)$.  Note that we have suppressed $N$ in the condition in $p_{vec}(\cdot)$, as $\mathbf{v}$ is a vector of dimension $d_v^N$, so the $N$ dependence is already implicitly encoded.  

\parbasic{\ccmapping{} and Semi-Equivariance} Let $\gamma$ be a function which takes as input the \complex{} consisting of both the \ligand{} $\ligsym$ and \receptor{} $\recsym$, and outputs a new vertex list $V'$ for the \ligand{} $\ligsym$:
\begin{equation}
    V' = \gamma(\ligsym, \recsym)
\end{equation}
We refer to $\gamma$ as a \textit{\ccmapping{}}.  A rigid body transformation $T \in E(3)$ consists of a rotation and translation; let the rotation be denoted as $T_{rot}$.  Then we say that $\gamma$ is \textit{rotation semi-equivariant} if
\begin{equation}
    \gamma(T_{rot}\ligsym, T\recsym) = T_{rot}\gamma(\ligsym, \recsym) \quad \text{for all } T \in E(3)
\end{equation}
where, as before, the action of $T$ on a graph is defined as in Section \ref{sec:notation}.  $\gamma$ is said to be \textit{permutation semi-equivariant} if
\begin{equation}
    \gamma(\pi \ligsym, \hat{\pi}\recsym) = \pi \gamma(\ligsym, \recsym) \quad \text{for all } \pi \in \mathbb{S}_N \text{ and } \hat{\pi} \in \mathbb{S}_{\hat{N}}
    \label{eq:gamma_permutation}
\end{equation}
where, as before, the action of the permutation on a graph is defined as in Section \ref{sec:notation}.  Note in the definitions of both types of semi-equivariance, the differing roles played by the \ligand{} and \receptor{}; as the equivariant behaviour only applies to the \ligand{}, we have used the term semi-equivariance.

\parbasic{\conditionalFlow{}} Let $\gamma$ be a \ccmapping{}.  If $\mathbf{v}$ is a vertex vector, define $\ligsym_{\mathbf{v}}$ to be the graph $\ligsym$ with the vertex set replaced by $\texttt{vec}^{-1}(\mathbf{v})$. Then the following ordinary differential equation is referred to as a \textit{\conditionalFlow{}}:
\begin{equation}
    \frac{d\mathbf{u}}{dt} = \texttt{vec}\left( \gamma(\ligsym_{\mathbf{u}} , \recsym) \right), \quad \text{with } \mathbf{u}(0) = \mathbf{z}
\end{equation}
where the initial condition $\mathbf{z} \sim \mathcal{N}(0, \mathbf{I})$ is a Gaussian random vector of dimension $d_v^N$, and the ODE is run until $t=1$.  $\mathbf{u}(1)$ is thus the output of the \conditionalFlow{}.

\parbasic{Vertex Distributions with Appropriate Invariance} We now have all of the necessary ingredients in order to construct a distribution $p_{vec}(\mathbf{v} | \recsym)$ which yields a vertex distribution $p(V | N, \recsym)$ that satisfies the invariance conditions that we require.  The following is our main result:

\begin{theorem}[Invariant Vertex Distribution]
Let $\mathbf{u}(1)$ be the output of a \conditionalFlow{} specified by the \ccmapping{} $\gamma$.  Let the mean position of the \receptor{} be given by $\bh{x}_{av} = \frac{1}{\hat{N}} \sum_{i=1}^{\hat{N}} \bh{x}_i$, and define the following quantities
\begin{equation}
    \alpha = \frac{N}{N + \hat{N}}
    \quad
    \Omega_{\recsym} = 
    \begin{bmatrix}
        \mathbf{I}_{3N} - \frac{\alpha}{N} \mathbf{1}_{N \times N} \otimes \mathbf{I}_3 & \mathbf{0} \\
        \mathbf{0} & \mathbf{I}_{d_h N}
    \end{bmatrix}
    \quad
    \omega_{\recsym} = 
    \begin{bmatrix}
        -(1-\alpha) \mathbf{1}_{N \times 1} \otimes \bh{x}_{av} \\
        \mathbf{0}
    \end{bmatrix}
\end{equation}
where $\otimes$ indicates the Kronecker product.  Finally, let $\mathbf{v} = \Omega_{\recsym}^{-1} \left( \mathbf{u}(1) - \omega_{\recsym} \right)$.  Suppose that $\gamma$ is both rotation semi-equivariant and permutation semi-equivariant.  Then the resulting distribution on $\mathbf{v}$, that is $p_{vec}(\mathbf{v} | \recsym)$, yields a vertex distribution $p(V | N, \recsym) = p_{vec}(\texttt{vec}(V) | \recsym)$ that satisfies the invariance conditions in Equation (\ref{eq:invariance}).
\end{theorem}

%\textbf{\textit{Proof:}} See Section \ref{sec:proof}.

\parbasic{Designing the \ccmapping{}} For the \ccmapping{}, we choose to use the \conditionalEGNN{}; that is, $V' = \gamma(\ligsym, \recsym)$ is given by $v'_i = (\mathbf{x}_i^L, \mathbf{h}_i^L)$, the output of the EGNN's final layer.
In practice, we use a slightly modified version of the foregoing, i.e. $v'_i = (\mathbf{x}_i^L-\mathbf{x}_i, \mathbf{h}_i^L)$, which we have found to converge well empirically. The rotation semi-equivariance of $\gamma$ (both versions - ordinary and displaced) follows straightforwardly from the rotation semi-equivariance of EGNNs and the rotation invariance of the \receptor{} signatures $\{ \bh{g}^\ell \}_{\ell=1}^L$.  Similarly, the permutation semi-equivariance follows from the permutation semi-equivariance of EGNNs and the permutation invariance of the \receptor{} signatures.

\parbasic{Loss Function}  The loss function and its optimization are implemented using standard techniques for continuous normalizing flows \citep{chen2018neural,grathwohl2018ffjord,chen2018continuous}.  If the feature vectors contain discrete variables, then techniques based on variational dequantization \citep{ho2019flow++} and argmax flows \citep{hoogeboom2021argmax} can be used, for ordinal and categorical features respectively.  This is parallel to the treatment in \citep{satorras2021flows}.

==> old/tab_validity_binding_1.tex <==
\begin{table}[tb]
    \begin{subtable}{.5\linewidth}
      \centering
        \begin{tabular}{ |c||c|c|c|} 
            \hline
            \multicolumn{4}{|c|}{\textbf{Validity}} \\
            \hline
            \multicolumn{2}{|c|}{Ours} & \multicolumn{2}{|c|}{GraphBP} \\
            \hline
            \multicolumn{2}{|c|}{99.87\%} & \multicolumn{2}{|c|}{99.75\%} \\
            \hline
            \hline
            \hline
            \multicolumn{4}{|c|}{\textbf{Bond Length Distribution}} \\
            \hline
            & Ref. Mols. & Ours & GraphBP \\
            \hline
            mean & 1.42 & 1.45 & 1.65 \\
            std & 0.08 & 0.10 & 0.95 \\
            \hline
        \end{tabular}
        \caption{Ligand validity and bond length distribution}
    \end{subtable}%
    \begin{subtable}{.5\linewidth}
      \centering
        \begin{tabular}{ |c||c|c|c|} 
            \hline
            \multicolumn{4}{|c|}{$\mathbf{\Delta}$\textbf{Binding}} \\
            \hline
            \multicolumn{2}{|c|}{Ours} & \multicolumn{2}{|c|}{GraphBP} \\
            \hline
            \multicolumn{2}{|c|}{35.7\%} & \multicolumn{2}{|c|}{22.76\%} \\
            \hline\hline\hline
            \multicolumn{4}{|c|}{\textbf{Predicted Affinity Distribution}} \\
            \hline
            & Ref. Mols. & Ours & GraphBP \\
            \hline
            mean & 5.09 & 4.56 & 4.31 \\
            std & 1.16 & 1.05 & 1.03 \\
            \hline
        \end{tabular}
        \caption{$\Delta$Binding and predicted affinity distribution}
    \end{subtable}
    \caption{Comparison of molecule validity and $\Delta$Binding between proposed method and GraphBP.}
    \label{tab:validity_binding}
\end{table}
